JUNO sensitivity to the annihilation of MeV dark matter in the galactic halo

We discuss JUNO sensitivity to the annihilation of MeV dark matter in the galactic halo via detecting inverse beta decay reactions of electron anti-neutrinos resulting from the annihilation. We study possible backgrounds to the signature, including the reactor neutrinos, diffuse supernova neutrino background, charged- and neutral-current interactions of atmospheric neutrinos, backgrounds from muon-induced fast neutrons and cosmogenic isotopes. A fiducial volume cut, as well as the pulse shape discrimination and the muon veto are applied to suppress the above backgrounds. It is shown that JUNO sensitivity to the thermally averaged dark matter annihilation rate in 10 years of exposure would be significantly better than the present-day best limit set by Super-Kamiokande and would be comparable to that expected by Hyper-Kamiokande.

==> Tables/Ch3_DM_EpDDist.tex <==
\begin{table}
\centering
\caption[The prompt energy cut and distance cut setting of inverse beta decay criteria.]{Prompt energy ($E_{\rm p}$) cut, prompt-delay distance ($\Delta D$) cut, and their efficiencies $\epsilon(E_{\rm p})$ and $\epsilon(\Delta D)$. }
\scalebox{0.85}{
\begin{tabular}{cccc}
\hline
$m_{\chi}$ & $E_{\rm p}$ cut range &  $\Delta D$ cut range & $\epsilon(E_{\rm p})$, $\epsilon(\Delta D)$ \\
\hline
15 MeV   &11-14 MeV & 0-370 mm & 0.995, \ 0.995\\
20 MeV   &16-19 MeV & 0-370 mm & 0.992, \ 0.995\\
25 MeV   &19-24 MeV & 0-430 mm & 0.989, \ 0.996\\
30 MeV   &25-29 MeV & 0-460 mm & 0.988, \ 0.994\\
35 MeV   &29-34 MeV & 0-500 mm & 0.983, \ 0.994\\
40 MeV   &33-39 MeV & 0-520 mm & 0.971, \ 0.995\\
45 MeV   &37-44 MeV & 0-580 mm & 0.971, \ 0.995\\
50 MeV   &41-48 MeV & 0-590 mm & 0.977, \ 0.997\\
55 MeV   &45-55 MeV & 0-650 mm & 0.970, \ 0.995\\
60 MeV   &49-58 MeV & 0-690 mm & 0.975, \ 0.995\\
65 MeV   &53-63 MeV & 0-730 mm & 0.963, \ 0.997\\
70 MeV   &57-68 MeV & 0-750 mm & 0.971, \ 0.995\\
75 MeV   &60-73 MeV & 0-800 mm & 0.969, \ 0.995\\
80 MeV   &63-78 MeV & 0-810 mm & 0.967, \ 0.994\\
85 MeV   &67-83 MeV & 0-880 mm & 0.962, \ 0.995\\
90 MeV   &69-87 MeV & 0-910 mm & 0.957, \ 0.996\\
95 MeV   &72-92 MeV & 0-960 mm & 0.963, \ 0.995\\
100 MeV  &75-97 MeV & 0-1050 mm & 0.954, \ 0.997\\
\hline \hline
\end{tabular}}
\end{table}

